Scheduling Algorithms for 5G Networks with Mid-haul Capacity Constraints

We consider a virtualized RAN architecture for 5G networks where the Remote Units are connected to a central unit via a mid-haul. To support high data rates, the midhaul is realized with a Passive Optical Network (PON). In this architecture, the data are stored at the central unit until the scheduler decides to transmit it through the mid-haul to an appropriate remote unit, and then over the air at the same slot. We study an optimal scheduling problem that arises in this context. This problem has two key features. First, multiple cells must be scheduled simultaneously for efficient operation. Second, the interplay between the time-varying wireless interface rates and the fixed capacity PON needs to be handled efficiently. In this paper, we take a comprehensive look at this resource allocation problem by formulating it as a utility-maximization problem. Using combinatorial techniques, we derive useful structural properties of the optimal allocation and utilize these results to design polynomial-time approximation algorithms and a pseudopolynomial-time optimal algorithm. Finally, we numerically compare the performance of the proposed algorithms to heuristics which are natural generalizations of the ubiquitous Proportional Fair algorithm.

==> FPTAS.tex <==
\subsection{An FPTAS for \textsf{Discrete}} \label{new_DP}

%In this section we derive an alternative DP, which readily yields an FPTAS for the problem \textsf{Single Slot}. We will be critically using Lemma 3 in this section. \\
%\begin{definition}[Under-utilization]
%	A RB $k$ is \emph{under-utilized} in the feasible solution $(\bm{x}, \bm{y})$ if $x_{jk}=1$ and $0< y_{jk} < \gamma_{jk}$. 
%\end{definition}
% 
% We have the following corollary from Lemma 3. 
% \begin{corollary} \label{uu}
% 	There exists an optimal solution $(\bm{x}^*, \bm{y}^*)$ to the problem \textsf{Single Slot}, such that there exists at most one under-utilized RB. 
% \end{corollary}
% Using corollary \ref{uu} we adopt the following strategy to solve the problem \textsf{Single Slot (SS)}: we take out one RB $k$ out of of a total of $K$ RBs as a potential underutilized RBs. We next solve the \textsf{SS} problem with $K-1$ RBs by replacing the constraint $y_{jk} \leq x_{jk} \gamma_{jk}$ by the equality constraint $y_{jk}=\gamma_{jk} x_{jk}$. Let's call this problem \textsf{Restricted Single Slot} (\textsf{RSS}$(k)$) with capacity constraint $C$. As can be seen in what follows, the problem \textsf{RSS} has flavor of the well-studied \textsf{Knapsack} problem. Once we have obtained a solution of \textsf{RSS}$(k)$, we augment this solution by filling up the rest of the capacity (up to $C$) as best as we can by the omitted RB $k$. By corollary $1$, we obtain the optimal solution by considering all $K$ possible RBs for omission and then taking the most profitable solution. \\
% From the above strategy, it is clear that an optimal solution to \textsf{RSS} translates to an optimal solution to \textsf{SS}. In the following, we develop a DP to solve the problem \textsf{RSS} optimally. 
% 
%  
 
%\subsection{An \textbf{FPTAS} for \textsf{Discrete} problem}
The above DP (DP-II)  has running time $\mathcal{O}(KC)$
which is  \emph{psuedo-polynomial} in the input size. However, using
appropriate scaling technique similar to the \textsf{Knapsack}
problem, it is possible to obtain \textbf{FPTAS} for
\textsf{Discrete}, which can in turn be used to obtain an
approximation for \textsf{Almost Discrete}, as the following Theorem shows. \\
  \begin{framed}
\begin{theorem}\label{d2ad}
From any optimal solution to \textsc{Discrete} we can construct a 
$\frac{1}{2}$-approximate solution to \textsc{Almost Discrete}. 
\end{theorem}
\end{framed}
Note that the total profit for any RB (irrespective of the PON capacity) is upper-bounded by $p_{\max}=\max_{j,k}Q_j\gamma_{jk}$. Fix an $\ve > 0$ and define a scaling factor $W= \frac{\ve p_{\max}}{K-1}$. Denote the profit obtained when the RB $k$ is assigned to the user $j$ by $p_{jk}$. Thus $p_{jk}=Q_j \gamma_{jk}$. \\
Now we consider the \textsf{RSS} problem for which $p'_{jk} = \lfloor \frac{p_{jk}}{W} \rfloor , \forall j,k$. This reduced problem, when solved by the DP algorithm has a table size of $\mathcal{O}(K \times \frac{K}{\ve})$ and the minimization step at each cell requires $\mathcal{O}(N)$ computation. Thus the overall scheme has run-time complexity of $\mathcal{O}(\frac{K^2N}{\ve})$. Next we bound the profit obtained by the reduced problem (after scaling $p'_{jk}$s up by a factor $W$) in terms of the profit of the optimal solution. 
%\subsection{Approximation Factor }   

Let us denote the approximate scaling algorithm $\mathcal{A}'$ and the optimal algorithm by \textsf{OPT}. Since $\mathcal{A}'$ is optimal for $p_{jk}'$, by definition we have 
\begin{eqnarray*}
	\sum_{jk}p_{jk}'(\mathcal{A'}) \geq \sum_{jk}p_{jk}'(\textsf{OPT}).
\end{eqnarray*}
Hence 
\begin{eqnarray*}
 	\textsf{Profit}(\mathcal{A}') &=& W\sum_{jk}p_{jk}'(\mathcal{A'})\\
 	&\geq&  W \sum_{jk}p_{jk}'(\textsf{OPT}) \\
 	&\geq& W \sum_{jk}\big(\frac{p_{jk}}{W}-1\big)(\textsf{OPT})\\
 	&= & \textsf{Profit}(\textsf{OPT})- W(K-1)\\
 	&= & \textsf{Profit}(\textsf{OPT})- \ve p_{\max} \\
 	&\geq & (1-\ve) \textsf{Profit}(\textsf{OPT}),
\end{eqnarray*} 
 where the last inequality follows because $\textsf{Profit}(\textsf{OPT}) \geq  p_{\max}$ \footnote{This is achievable because we have filtered the input to allow only those $\gamma_{jk}$s such that $C\geq \max_{j} \gamma_{jk}$.}.
% \subsection{$\frac{1}{2}-\ve$ approximation FPTAS for \textsc{Almost Discrete}}

Combining the FPTAS for \textsc{Discrete} with the strategy $\pi$ from
Theorem~\ref{d2ad}, we readily obtain a $\frac{1}{2}-\ve$ FPTAS for \textsc{Almost Discrete}. 
 
 
% \subsection{Avoiding solving \textsf{SS} altogether}
% It is also possible to avoid solving SS and get a $2$ approximation algorithm from \textsf{RSS} itself. Consider these two schemes: Allocate the best RB to the best user (max-yield) to obtain a profit of $p_{\max}=\max_j Q_j \gamma_{jk}$ \footnote{We assume $\max_{j,k}\gamma_{jk} \leq C$, for simplicity.} And solving the DP above and taking the best of the above solutions (not necessarily filling up the rest of the capacity). In the optimal solution, at least one of them would be more than half of the optimal (since optimal solution comprises of RSS plus a fractional part). This constitutes a half-approximation algorithm.  
% 
% 
 
 
 
 
 
 
 
 

==> pd.tex <==
\section{A Primal-Dual Formulation}
The dual of the LP version of the optimization problem may be written down as follows:
\begin{eqnarray} \label{dual}
	\min \sum_k z_k + \lambda C
\end{eqnarray}
Subject to, 
\begin{eqnarray}
	\lambda + \mu_{jk} &\geq& Q_{j}\\
	-\gamma_{jk} \mu_{jk} + z_k &\geq& 0\\
	\lambda, z_k, \mu_{jk} &\geq& 0 
\end{eqnarray}
